Ab Initio Quantum Monte Carlo Simulations of the Uniform Electron Gas without Fixed Nodes II: Unpolarized Case

In a recent publication [S. Groth \textit{et al.}, PRB (2016)], we have shown that the combination of two novel complementary quantum Monte Carlo approaches, namely configuration path integral Monte Carlo (CPIMC) [T. Schoof \textit{et al.}, PRL \textbf{115}, 130402 (2015)] and permutation blocking path integral Monte Carlo (PB-PIMC) [T. Dornheim \textit{et al.}, NJP \textbf{17}, 073017 (2015)], allows for the accurate computation of thermodynamic properties of the spin-polarized uniform electron gas (UEG) over a wide range of temperatures and densities without the fixed-node approximation. In the present work, we extend this concept to the unpolarized case, which requires non-trivial enhancements that we describe in detail. We compare our new simulation results with recent restricted path integral Monte Carlo data [E. Brown \textit{et al}., PRL \textbf{110}, 146405 (2013)] for different energy contributions and pair distribution functions and find, for the exchange correlation energy, overall better agreement than for the spin-polarized case, while the separate kinetic and potential contributions substantially deviate.

==> cpimc_sketch.tikz.tex <==
%\begin{tikzpicture}[xscale=0.74, yscale=0.4]
\begin{tikzpicture}[xscale=0.71, yscale=0.45]
\newcommand{\xrange}{10}
\newcommand{\yrange}{1}
\newcommand{\taueins}{\xrange*0.3}
\newcommand{\tauzwei}{\xrange*0.45}
\newcommand{\taudrei}{\xrange*0.8}
%\newcommand{\tauvier}{\xrange*0.7}
%\newcommand{\taufuenf}{\xrange*0.9}
\newcommand{\zero}{\yrange*1}
\newcommand{\eins}{\yrange*2}
\newcommand{\zwei}{\yrange*3}
\newcommand{\drei}{\yrange*4}
\newcommand{\vier}{\yrange*5}
\newcommand{\fuenf}{\yrange*6}
\newcommand{\sechs}{\yrange*7}
\newcommand{\sieben}{\yrange*8}
\newcommand{\acht}{\yrange*9}

%draw coordinate system
\draw[->] (0,0) -- +(\xrange+0.5*\xrange/20,0) coordinate (xlabel);
\draw[->] (0,0) -- +(0,\yrange*10) coordinate (ylabel);
\foreach \i in {0,...,8} {
	\draw (-0.1,\i*\yrange+\yrange) node[left] {$\i$} -- (0.1,\i*\yrange+\yrange);
}

%draw spins 
\foreach \i in {0,2,4,6,8} {
	\node at (\xrange+0.3,\i*\yrange+\yrange) {$\uparrow$};
}
\foreach \i in {1,3,5,7} {
	\node at (\xrange+0.3,\i*\yrange+\yrange) {$\downarrow$};
}
\node[rotate=270] at (\xrange+0.8,5*\yrange) {spin projection $\sigma_i$};

\foreach \i/\l in {\taueins/$\tau_1$,\tauzwei/$\tau_2$,\taudrei/$\tau_3$} {
\draw (\i,0.1) -- (\i,-0.1) node[below] {\l};
}
\draw (0,0.1) -- (0,-0.1) node[below] {$0$};
\draw (\xrange,0.1) -- (\xrange,-0.1) node[below] {$\beta$};
\node at (0.5*\xrange,-1.5) {imaginary time $\tau$};
\node[rotate=90] at (-0.9,5*\yrange) {orbital $i$};

%draw empty sites
\foreach \i in {1,...,9} {
\draw[semithick,dotted] (0,\i*\yrange) -- (\xrange,\i*\yrange);
}

%\draw[dashed] (\taudrei + \tauvier/2.0-\taudrei/2.0 -0.25,0.5) rectangle (\taudrei + \tauvier/2-\taudrei/2+0.25,\yrange*6.5);
\draw[dashed] (\tauzwei+2.0,0.5) rectangle (\tauzwei+2.75,\acht+0.5);
\node at (\tauzwei + 3.0,\acht+1.3) {$|\{n^{(2)}\}\rangle=|001100110\ldots\rangle$};

% 
\begin{scope}[thick]
\draw (0,\zero) -| (\taueins,\zwei) -| (\taudrei,\zero) -- (\xrange,\zero);
\draw (0,\eins) -| (\tauzwei,\sieben) -| (\taudrei,\eins) -- (\xrange,\eins);
\draw (0,\drei) -| (\taueins,\fuenf) -| (\tauzwei,\drei) -- (\xrange,\drei);
\draw (\taueins, \drei) -- (\taueins, \zwei);
\draw (0,\sechs) -- (\xrange,\sechs);
%\draw (\taudrei, \eins) -- (\taudrei, \zwei);
 \end{scope}
 
 \node at (\taueins, \fuenf+\yrange-0.5) { $s_1 =(2,5,0,3)$};
 %\node at (\taufuenf, \fuenf+\yrange) { $s_5 =(1,5)$};


\end{tikzpicture}

